On the Cost of Concurrency in Transactional Memory

Traditional techniques for synchronization are based on \emph{locking} that provides threads with exclusive access to shared data. \emph{Coarse-grained} locking typically forces threads to access large amounts of data sequentially and, thus, does not fully exploit hardware concurrency. Program-specific \emph{fine-grained} locking or \emph{non-blocking} (\emph{i.e.}, not using locks) synchronization, on the other hand, is a dark art to most programmers and trusted to the wisdom of a few computing experts. Thus, it is appealing to seek a middle ground between these two extremes: a synchronization mechanism that relieves the programmer of the overhead of reasoning about data conflicts that may arise from concurrent operations without severely limiting the program's performance. The \emph{Transactional Memory (TM)} abstraction is proposed as such a mechanism: it intends to combine an easy-to-use programming interface with an efficient utilization of the concurrent-computing abilities provided by multicore architectures. TM allows the programmer to \emph{speculatively} execute sequences of shared-memory operations as \emph{atomic transactions} with \emph{all-or-nothing} semantics: the transaction can either \emph{commit}, in which case it appears as executed sequentially, or \emph{abort}, in which case its update operations do not take effect. Thus, the programmer can design software having only sequential semantics in mind and let TM take care, at run-time, of resolving the conflicts in concurrent executions. Intuitively, we want TMs to allow for as much \emph{concurrency} as possible: in the absence of severe data conflicts, transactions should be able to progress in parallel. But what are the inherent costs associated with providing high degrees of concurrency in TMs? This is the central question of the thesis.

==> p3disc.tex <==
%!TEX root = part3.tex
\chapter{Discussion of Part~\ref{part:three}}
\label{ch:p3disc}
%
The complexity of TM is parametrized by several measures: 
TM, TM-progress and TM-liveness, 
DAP and invisible read assumptions, bound on the number of versions that can be maintained 
at any prefix of an execution and whether the TM can be implemented from read-write base objects.
We conclude Part~\ref{part:three} by providing a summary of known TM complexity bounds, relation to the
TM bounds presented in the thesis, if any, and overview some interesting open questions.
%
\section{Summary of TM complexity bounds and open questions}
\label{sec:p3summary}
%
\vspace{1mm}\noindent\textbf{Blocking TMs.}

\vspace{1mm}\noindent\textbf{Non-blocking TMs.}
Guerraoui and Kapalka~\cite{tm-book} proved that it is impossible to implement
strict DAP strictly serializable TMs in $\mathcal{OF}$. 
They also proved that a strict serializable TM that provides OF TM-progress and
wait-free TM-liveness cannot be implemented using only read and write primitives.

\vspace{1mm}\noindent\textbf{Partially non-blocking TMs.}
Attiya \emph{et al.}~\cite{AHM09} showed that it is impossible to implement 
weak DAP strictly serializable TMs in $\mathcal{RWF}$ 
if read-only transactions may only apply trivial primitives to base objects.
Attiya et al.~\cite{AHM09} also considered a stronger ``disjoint-access'' property, 
called simply DAP, referring to the
original definition proposed Israeli and
Rappoport~\cite{israeli-disjoint}.
In DAP,  two transactions are allowed to \emph{concurrently access} (even
for reading) the same base object only if they are disjoint-access.
For an $n$-process DAP TM implementation,  it is shown in~\cite{AHM09}
that a read-only transaction must
perform at least $n-3$ writes. 
Our lower bound in Theorem~\ref{th:rwf} is strictly stronger than the one in~\cite{AHM09}, as
it assumes only weak DAP,
considers a more precise RAW/AWAR metric, 
and does not depend on the number of processes in the system.
(Technically, the last point follows from the fact that the execution
constructed in the proof of Theorem~\ref{th:rwf}
uses only  $3$ concurrent processes.)
Thus, the theorem subsumes the two lower bounds of~\cite{AHM09} within a single proof.

Perelman \emph{et al.}, considered the closely related (to $\mathcal{RWF}$) class of 
\emph{mv-permissive} TMs:
a transaction can only be aborted if it is an \emph{updating} transaction that conflicts with another
\emph{updating} transaction~\cite{PFK10}.
$\mathcal{RWF}$ is incomparable
with the class of mv-permissive TMs. On the one hand,
mv-permissiveness guarantees that read-only transactions never abort, but does not imply that they commit
in a wait-free manner.  
On the other hand, $\mathcal{RWF}$ allows an
updating transaction to abort in the presence of a concurrent
read-only transaction, which is disallowed by mv-permissive TMs.       
Observe that, technically, mv-permissiveness is a blocking TM-progress condition, although when used in conjunction with
wait-free TM-liveness, it is a partially non-blocking TM-progress condition that is strictly stronger than $\mathcal{RWF}$.

Assuming starvation-free TM-liveness,
\cite{PFK10} showed that 
implementing a weak DAP strictly serializable mv-permissive TM is impossible.
In the thesis, we showed that strictly serializable TMs in $\mathcal{RWF}$ cannot provide strict DAP, but proving
the impossibility result assuming weak DAP remains an interesting open question.
%[[PK what do you mean ``not subject''? there is no proof, right?
%While $\mathcal{RWF}$ is not subject to this
%impossibility, it is impossible to implement strict DAP implementations in $\mathcal{RWF}$.
%]]
% In principle, the class of TMs considered in~\cite{PFK10} is a proper subset of our
% $\mathcal{RWF}$.

\cite{PFK10} also proved that mv-permissive TMs cannot be \emph{online
  space optimal}, \emph{i.e.}, no mv-permissive TM can keep the minimum number of old object
versions for any TM history. 
Our result on the space complexity of implementations in $\mathcal{RWF}$ that use invisible reads (Theorem~\ref{th:inv})
is different since it proves that the implementation must maintain an unbounded number of versions
of every t-object. 
Our proof technique can however be used to show that 
mv-permissive TMs considered in \cite{PFK10} should also maintain unbounded number of versions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> p3overview.tex <==
\chapter{Overview of Part~\ref{part:three}}
\label{ch:p3overview}
%
\section{Introduction}
\label{sec:p3intro}
%
In Part~\ref{part:one}, we formalized the notion of \emph{safe} TM implementations. But what is the complexity
of safe TM implementations that provide meaningful progress guarantees? In Part~\ref{part:three}, we present several
complexity lower and upper bounds that help answer this question.

\vspace{1mm}\noindent\textbf{Blocking TMs.}
We begin by studying TM implementations that provide no non-blocking progress guarantees for transactions
and typically allow a transaction to \emph{block} or abort in \emph{conflicting} executions.

We start by presenting complexity bounds for \emph{single-lock} TMs that satisfy sequential TM-progress.
We show that a read-only transaction in an opaque (and resp. strictly serializable) TM featured with \emph{weak disjoint-access parallelism (DAP)}, 
\emph{weak invisible reads} and ICF TM-liveness must \emph{incrementally} validate
every next read operation. This results in a quadratic (and resp. linear) (in the size of the transaction's read
set) step-complexity lower bound.
Informally, weak DAP means that two transactions
can \emph{contend} (\emph{i.e.}, both access the base object and at least one modifies it) 
on a common base object only if their data 
sets are connected in the \emph{conflict graph}, capturing 
data-set overlaps among all concurrent transactions.
Weak read invisibility allows t-read operations of a transaction
$T$ to be ``visible'', \emph{i.e.}, write to base objects, only if $T$ is concurrent with
another transaction.
We then show that even single-lock TMs must perform a 
RAW (read-after-write) or AWAR (atomic-write-after-read)
pattern~\cite{AGK11-popl}. The RAW/AWAR patterns capture the amount of ``expensive
synchronization'', \emph{i.e.}, the number of costly conditional primitives
or memory barriers~\cite{AdveG96} incurred by the
implementation.

We turn our focus to \emph{progressive} TM implementations which allow a transaction to be aborted only
on read-write conflicts with concurrent transactions.
We introduce a new metric called \emph{protected data size}
that, intuitively, captures the amount of data that a transaction 
must exclusively control at some point of its execution. 
All progressive TM implementations we are aware of 
(see, \emph{e.g.}, an overview in~\cite{GK09-progressiveness})
use locks or timing assumptions to give an updating transaction exclusive access  
to all objects in its write set at some point of its execution.
For example, lock-based progressive implementations like \emph{TL}~\cite{DStransaction06} and \emph{TL2}~\cite{DSS06} require that a
transaction grabs all locks on its write set
before updating  the corresponding base objects.    
Our results show that this is an inherent price to pay for
providing progressive concurrency: every committed transaction in a progressive and 
\emph{strict DAP} (a restriction of weak DAP which ensures that two transactions contend on a common base object only if they access
a common t-object) TM implementation 
must, at some point of its execution, protect every t-object 
in its write set.
We then present a very cheap progressive opaque strict DAP TM implementation from read-write base objects
with constant expensive synchronization and constant \emph{memory stall} complexities.
Intuitively, the stall metric captures the fact that the time a process might have to spend before it applies a 
primitive on a base object
can be proportional to the number of processes that try to update the
object concurrently.  

We then prove that in any \emph{strongly progressive} strictly serializable TM
implementation that accesses the shared memory with \emph{read}, \emph{write} and \emph{conditional}
primitives, such as \emph{compare-and-swap} and
\emph{load-linked/store-conditional}, 
the total number of \emph{remote memory references} (RMRs) 
that take place in an execution of a progressive TM in which $n$
concurrent processes perform transactions on a single t-object might
reach $\Omega(n \log n)$. 
The result is obtained via a reduction to an analogous lower bound for
mutual exclusion~\cite{rmr-mutex}.
In the reduction, we show that any TM with the above properties can be
used to implement a \emph{deadlock-free} mutual exclusion, employing
transactional operations on only one t-object and incurring a constant RMR overhead. 
The lower bound applies to RMRs in both the \emph{cache-coherent (CC)} and
\emph{distributed shared memory (DSM)} models, and it appears to be the first RMR complexity
lower bound for transactional memory.
We also present a constant expensive synchronization strongly progressive TM implementation from read-write base objects.
Our implementation provides \emph{starvation-free} TM-liveness, thus showing one means of circumventing the lower bound
of Rachid \emph{et al.}~\cite{tm-book} who proved the impossibility of implementing strongly progressive
strictly serializable TMs providing \emph{wait-free} TM-liveness from read-write base objects.

We conclude our study of blocking TMs by establishing a linear (in the transaction's data set size)
separation between the worst-case transaction expensive synchronization complexity of strongly progressive TMs and 
\emph{permissive} TMs that allow a transaction to abort only if committing it would violate opacity.

\vspace{1mm}\noindent\textbf{Non-blocking TMs.}
We present several complexity bounds for non-blocking TMs exemplified by
\emph{obstruction-freedom}, possibly the weakest non-blocking
progress condition~\cite{HLM03,HS11-progress}.

We first establish that it is impossible to
implement a strictly serializable obstruction-free TM that provides both weak DAP and \emph{read invisibility}.
Read invisibility, as the name suggests is stronger than weak read invisibility and requires
that a transaction cannot reveal any information about its read set to
other transactions and hence, no reading transaction can cause another transaction to abort. 
Indeed, popular obstruction-free TMs like \emph{DSTM}~\cite{HLM+03} and \emph{FSTM}~\cite{fraser} are weak DAP, but
use \emph{visible} reads for aborting pending writing transactions.
Secondly, we show that a t-read operation in a $n$-process strictly serializable obstruction-free TM
implementation may incur $\Omega(n)$ stalls.
Thirdly, we prove that any \emph{read-write (RW) DAP} opaque
obstruction-free 
TM implementation has an execution in which a
read-only transaction incurs $\Omega(n)$ non-overlapping \emph{RAWs} or \emph{AWARs}. 
RW DAP, a restriction of weak DAP and a relaxation of strict DAP,
defines the conflict graph based 
on the \emph{write-set overlaps} among concurrent transactions and is satisfied by popular
obstruction-free implementations~\cite{HLM+03,fraser,nztm}. 
Finally, we show that there exists a considerable complexity gap between blocking (\emph{i.e.}, progressive) and 
non-blocking (\emph{i.e.}, obstruction-free) TM implementations.

\vspace{1mm}\noindent\textbf{Partially non-blocking TMs.}
It is easy to see that \emph{dynamic} TMs where
the patterns in which transactions access t-objects 
are not known in advance do not allow for
\emph{wait-free} TMs~\cite{tm-book}, \emph{i.e.}, every transaction must commit in a finite number of steps of the process
executing it,  regardless of the behavior of concurrent
processes.
Suppose that a transaction
$T_1$ reads t-object $X$, then a concurrent transaction $T_2$ reads
t-object $Y$, writes to $X$ and commits, and finally $T_2$ writes to
$Y$. 
Since $T_1$ has read the ``old'' value in $X$ and $T_2$ has read the
``old'' value  in $Y$, there is no way to commit $T_1$ and order the
two transactions in a sequential execution.   
As this scenario can be repeated arbitrarily often, even the weaker guarantee of \emph{local progress} that only requires that
each transaction \emph{eventually} commits if repeated
sufficiently often, cannot be ensured by \emph{any} strictly
serializable TM implementation,
regardless of the base objects it
uses~\cite{bushkov2012}.\footnote{Note that the counter-example would
  not work if we imagine that 
  the program encapsulated in a transaction can be known in
  advance. However, in the thesis, we consider the conventional
  dynamic TM programming model.}              
 
But can we ensure that at least \emph{some} transactions commit wait-free and what are the inherent costs?
%
%Furthermore, the TM implementation must provide nontrivial progress for transactions i.e. specify the conditions
%under which a transaction cannot be aborted.
It is often argued that many realistic workloads are
\emph{read-dominated}: the proportion of read-only transactions is
higher than that of updating ones, or read-only transactions have much
larger data sets than updating ones~\cite{stmbench7, Attiya09-tmread}. 
%\textbf{Is this true? Any   references?SR: is this ok?}
Therefore, it seems natural to require that read-only transactions
commit wait-free. Since we are interested in complexity lower bounds, we require that
updating transaction provide only sequential TM-progress. 

First, we focus on strictly serializable TMs with the above TM-progress conditions 
that use invisible reads.
We show that this requirement results in maintaining unbounded sets of versions
for every data item, \emph{i.e.}, such implementations 
may not be practical due to their space complexity. 
Secondly, we prove that strictly serializable TMs with these progress conditions
cannot ensure strict DAP. 
Thus, two transactions that access mutually disjoint data sets may prevent each other from committing.
Thirdly, for weak DAP TMs, we show that a read-only transaction (with
an arbitrarily large read
set) must sometimes perform at least one
expensive synchronization pattern~\cite{AGK11-popl} per t-read
operation, \emph{i.e.},
the expensive synchronization complexity of a read-only transaction is linear in
the size of its data set.     

\vspace{1mm}\noindent\textbf{Roadmap of Part~\ref{part:three}.}
In Chapter~\ref{ch:p3c1}, we introduce the TM properties of invisible reads and disjoint-access parallelism.
In Chapter~\ref{ch:p3c2}, we study complexity bounds for blocking TMs, in
Chapter~\ref{ch:p3c3} for non-blocking TMs and in Chapter~\ref{ch:p3c4} for partially non-blocking TMs.
We conclude in Chapter~\ref{p3disc} with a summary of TM bounds and interesting open questions.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
%
\section{Complexity metrics}
\label{sec:complexity}
%
We now present an overview of some of the TM complexity metrics we consider in the thesis.

\vspace{1mm}\noindent\textbf{RAW/AWAR metric.}
Attiya \emph{et al.} identified two common expensive synchronization patterns that frequently arise in
the design of concurrent algorithms: \emph{read-after-write (RAW) or atomic write-after-read (AWAR)}~\cite{AGK11-popl,McKenney10}
and showed that it is 
impossible to derive RAW/AWAR-free implementations of
a wide class of data types that include \emph{sets}, \emph{queues} and \emph{deadlock-free mutual exclusion}.

Intuitively, RAW (read-after-write) or AWAR (atomic-write-after-read)
patterns~\cite{AGK11-popl} capture the amount of ``expensive
synchronization'', \emph{i.e.}, the number of costly conditional primitives
or memory barriers~\cite{AdveG96} incurred by the
implementation.
The metric appears to be more practically relevant than simple
step complexity, as it accounts for expensive cache-coherence operations or conditional instructions.
Detailed coverage on memory fences and the RAW/AWAR metric can be found in \cite{McKenney10}.

A \emph{RAW} (read-after-write) pattern  performed by a transaction
$T_k$ in an execution $\pi$ 
%$\exists i,j; 0 \leq i < j < |\pi|$
is a pair of its events $e$ and $e'$, such that: (1) $e$ is a write to a
base object $b$ by $T_k$, 
(2) $e'$ is a subsequent read of a base object $b'\neq b$ by $T_k$, and 
(3) no event on $b$ by $T_k$ takes place between $e$ and $e'$. 
In this paper, we are concerned only with \emph{non-overlapping} RAWs,
\emph{i.e.}, the read performed by one RAW precedes the write 
performed by the other RAW.
%
An \emph{AWAR} (atomic-write-after-read) pattern $e$ in an execution
$\pi\cdot e$ is a nontrivial rmw event on an object $b$ which
atomically returns the value of $b$ (resulting after $\pi$) and updates $b$ with a
new value, {\em e.g.}, a successful \emph{compare-and-swap}.  

\vspace{1mm}\noindent\textbf{Stall complexity.}
Intuitively, the stall metric captures the fact that the time a process might have to spend before it applies a 
primitive on a base object can be proportional to the number of processes that try to update the object concurrently.  

Let $M$ be any TM implementation.
Let $e$ be an event applied by process $p$ to a base object $b$ as it performs a transaction $T$ during an execution $E$ of $M$.
Let $E=\alpha\cdot e_1\cdots e_m \cdot e \cdot \beta$ be an execution of $M$, where $\alpha$ and $\beta$ are execution 
fragments and $e_1\cdots e_m$
is a maximal sequence of $m\geq 1$ consecutive nontrivial events by distinct distinct processes other than $p$ that access $b$.
Then, we say that $T$ incurs $m$ \emph{memory stalls in $E$ on account of $e$}.
The \emph{number of memory stalls incurred by $T$ in $E$} is the sum of memory stalls incurred by all events of $T$ in $E$~\cite{G05,AGHK09}.

In the thesis, we adopt the following definition of a \emph{k-stall execution} from \cite{AGHK09,G05}.
%
\begin{definition}
\label{def:stalls}
%
An execution $\alpha\cdot \sigma_1 \cdots \sigma_i$ is a $k$-stall execution for t-operation $op$ executed by process $p$ if
%
\begin{itemize}
\item 
$\alpha$ is $p$-free,
\item
there are distinct base objects $b_1,\ldots , b_i$ and disjoint sets of processes $S_1,\ldots , S_i$
whose union does not include $p$
and has cardinality $k$ such that, for $j=1,\ldots i $,
%
\begin{itemize}
\item
each process in $S_j$ has an enabled nontrivial event about to access base object $b_j$ after $\alpha$, and
\item
in $\sigma_j$, $p$ applies events by itself until it is the first about to apply an event to $b_j$,
then each of the processes in $S_j$ applies an event that accesses $b_j$, and finally, $p$ applies an event that accesses $b_j$,
\end{itemize}
\item
$p$ invokes exactly one t-operation $op$ in the execution fragment $\sigma_1\cdots \sigma_i$
\item
$\sigma_1\cdots \sigma_i$ contains no events of processes not in $(\{p\}\cup S_1\cup \cdots \cup S_i)$
\item
in every $(\{p\}\cup S_1\cup \cdots \cup S_i)$-free execution fragment that extends $\alpha$, 
no process applies a nontrivial event to any base object accessed in $\sigma_1 \cdots \sigma_i$.
\end{itemize}
%
\end{definition}
%
Observe that in a $k$-stall execution $E$ for t-operation $op$, the number of memory stalls incurred by $op$
in $E$ is $k$.

The following lemma will be of use in our proofs.
%
\begin{lemma}
\label{lm:stalls}
Let $\alpha\cdot \sigma_1 \cdots \sigma_i$ be a $k$-stall execution for t-operation $op$ executed by process $p$.
Then, $\alpha\cdot \sigma_1 \cdots \sigma_i$ is indistinguishable to $p$ from a step contention-free execution~\cite{AGHK09}.
\end{lemma}
%
\vspace{1mm}\noindent\textbf{Remote memory references(RMR)~\cite{rmr-mutex}.}
Accesses to memory locations (\emph{i.e.} base objects) that are \emph{remote} to a given process
are often magnitudes of times slower than a \emph{local} access of the base object.
Thus, the performance of concurrent implementations in the shared memory model may depend on the number on the number
of \emph{references} made to the remote base objects.

In the \emph{cache-coherent (CC) shared memory}, each process maintains \emph{local}
copies of shared base objects inside its cache, whose consistency is ensured by a coherence protocol.
Informally, we say that an access to a base object $b$ is \emph{remote} to a process $p$ and 
causes a \emph{remote memory reference (RMR)} if $p$'s cache contains a 
cached copy of the object that is out of date or \emph{invalidated}; otherwise the access is \emph{local}.

In the \emph{write-through (CC) protocol}, to read a base object $b$, process $p$ must have a cached copy of $b$ that
has not been invalidated since its previous read. Otherwise, $p$ incurs a RMR. 
To write to $b$, $p$ causes a RMR that invalidates all cached copies
of $b$ and writes to the main memory.

In the \emph{write-back (CC) protocol}, $p$ reads a base object $b$ without causing a RMR if it holds a cached copy of $b$
in shared or exclusive mode; otherwise the access of $b$ causes a RMR that (1) 
invalidates all copies of $b$ held in exclusive mode, and writing $b$ back to the main memory,
(2) creates a cached copy of $b$ in shared mode.
Process $p$ can write to $b$ without causing a RMR if it holds a copy of $b$ in exclusive mode; otherwise
$p$ causes a RMR that invalidates all cached copies of $b$ and creates a cached copy of $b$ in exclusive mode.

In the \emph{distributed shared memory (DSM)}, each register is forever assigned to a single process and it
\emph{remote} to the others. Any access of a remote register causes a RMR.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
